Automatic Differentiation for ML-family languages: correctness via logical relations

We give a simple, direct and reusable logical relations technique for languages with term and type recursion and partially defined differentiable functions. We demonstrate it by working out the case of Automatic Differentiation (AD) correctness: namely, we present a correctness proof of a dual numbers style AD code transformation for realistic functional languages in the ML-family. We also show how this code transformation provides us with correct forward- and reverse-mode AD. The starting point is to interpret a functional programming language as a suitable freely generated categorical structure. In this setting, by the universal property of the syntactic categorical structure, the dual numbers AD code transformation and the basic $\omega$-cpo semantics arise as structure preserving functors. The proof follows, then, by a novel logical relations argument. The key to much of our contribution is a powerful monadic logical relations technique for term recursion and recursive types. It provides us with a semantic correctness proof based on a simple approach for denotational semantics, making use only of the very basic concrete model of $\omega$-cpos.

==> TEX/Assignment-LR.tex <==
\small 
\[
\begin{array}{c}
\semLR{n,k}{\op } : \semLR{n, k}{\reals  }^m \to \monadLR{n,k}{\semLR{n,k}{\reals  }} , \quad
	\semLR{n,k}{\cnst c } : \lift{\terminall}  \to  \semLR{n,k}{\reals  } , \quad
	\semLR{n, k}{\tSign } : \semLR{n, k}{\reals  } \to  \monadLR{n, k}{\lift{\terminall }\sqcup\lift{\terminall} },
\end{array}
\] \\
\normalsize for each primitive operation  $\op\in\Op_m$ ($m\in\NN$) and each constant  $c\in \RRsyntax$.


==> TEX/DomainSemantics.tex <==
\section{Concrete models: \wcpos}\label{sec:owcpos-enriched-stuff}
The aim of this section is to establish a class of concrete $CBV$ models.
We denote by $ \wCpo $ the usual category of \wcpos. The objects of  $ \wCpo $ are the
partially ordered sets with colimits of $\ww$-chains, while the morphisms are functors preserving these colimits.

It is well known that $ \wCpo $ is cartesian closed\footnote{In fact, it is locally presentable and its internal hom $X\Rightarrow Y$ is given by using the order $f\leq g$ if and only if $\forall x\in X.f(x)\leq_Y g(x)$ on the homset $\wCpo(X,Y)$. See, for example, \cite{vakar2019domain}.}. 
We can, then, get the enriched versions of the definitions in Section \ref{sec:basic-categorical-semantics}.
A $\wCpo $-category 
$\catV $ is $\wCpo $-bicartesian closed if $\catV $ has finite products and coproducts and, moreover, 
for each $Y\in\catV $, the $ \wCpo $-functor 
\begin{equation}
	\left( Y\times -\right) : \catV\to\catV 
\end{equation}
has a right $\wCpo $-adjoint, which we will denote by the usual notation $\expo{Y}{-}$ of exponentials.

Recall that, in this context, a   $ \wCpo $-monad is strong if it is equipped with a $\wCpo$-natural
transformation 
\begin{equation}
	\strengthT : -\times T(-)\longrightarrow T(-\times -),
\end{equation}
called strength, such that the diagrams
\begin{equation}
	\diag{strong-monad-compatibility-associativity}\quad\diag{strong-monad-compatibility-identity}
\end{equation}
\begin{equation}
	\diag{strong-monad-compatibility-multiplication}\quad\diag{strong-monad-compatibility-unit}
\end{equation}
commute, for any $\left( W,Y,Z\right)\in\catV\times\catV\times\catV $.




 A pair $\left( \catV , \monadT \right) $, where  $\catV$ is an $ \wCpo $-enriched category and $\monadT$ is a strong $ \wCpo $-monad, is called a \textit{$CBV$ $\wCpo$-pair}. 
 
Let $\left( \catV , \monadT \right) $ be such a pair. We denote by
\begin{equation}
 -\otimes - : \catV\times\catC \to \catC
\end{equation}
 the $\catV$-tensor product in $\catC$. Recall that, if $ J: \catV\to\catC $ is the corresponding $\catV$-enriched universal Kleisli functor, $-\otimes J(-) = J\left( -\times - \right) $.  
  For any $(W,Y,Z)\in \catV $, we have that, given a morphism $f: Z\otimes W\to W\sqcup Y $ of $\catC $, for each $x\in Z $,  we can define
\begin{equation}
	\underline{f}_x: \ehomC{ W}{Y} \to \ehomC{ W}{Y}, \qquad h\mapsto \pairL\ID _W ,  f_x \pairR\circ h  
\end{equation}  
$\ehomC{ W}{Y}$
  where $f_x $ is $\overline{f}(x) $ where $\overline{f}: Z\to \ihomC{W}{W\sqcup Y} $ is the $\catV $-morphism corresponding to $f$. The least fixed point 
  
\begin{equation}
 \ehomC{Z\otimes W}{W\sqcup Y} \to\ehomC{Z\otimes W}{Y} 
\end{equation} 




==> TEX/InitialAlgebras.tex <==
\section{Initial algebras, again}\label{app:initial-algebras-again}


==> TEX/app-Non-used-Material-on-Recursive-Types.tex <==
\section{Unused material on recursive types}\label{app:I-did-not-used-recursive-types}



%Every embedding $u : A \pembedding B$ in a partial map category with axiom
%\pMapEnrichment{} is a total map $u : A \to
%B$~\cite[Prop.~5.4.2]{fiore:thesis}.

An \emph{\wchain{} of ep-pairs} $\pair{\seq[n \in
	\NN]{A_n}}{\seq[n \in \NN]{a_n}}$ in $\catC$
consists of a countable sequence of objects $A_n$ and a countable
sequence of ep-pairs $a_n : A_n \epto A_{n+1}$. A \emph{bilimit}
$\pair Dd$ of such an \wchain{} consists of an object $D$ and a
countable sequence of ep-pairs $\smash{d_n : A_n \epto D}$ such that,
for all $n \in \NN$, $\smash{d_{n+1}\circ a_n = d_n}$, and
$\smash{\vee_{n \in \NN} \emb d_n\circ  \prj d_n   =
	\id[D]}$. The celebrated \emph{limit-colimit
	coincidence}~\cite{smyth-plotkin:rde} states that the bilimit
structure is equivalent to a colimit structure $\pair{D}{\emb d}$ for
$\pair*{\seq{A_n}}{\seq{\emb a_n}}$, in which case $\prj d_n$ are
uniquely determined, and similarly equivalent to a limit structure
$\pair*{D}{\prj d}$ for $\pair*{\seq{A_n}}{\seq{\prj a_n}}$, in
which case $\emb d_n$ are uniquely determined.

A \emph{zero object} is an object that is both initial and
terminal. A zero object in an $\wCpo$-category~is an \emph{ep-zero object}  if
every morphism into it is a projection and every
morphism out of it is an~embedding.

A \emph{bilimit compact category} is an $\wCpo$-category $\catC$
with an ep-zero and ep-pair \wchain{} bilimits.
When $ \catC$ is bilimit compact and $\catD$ is some $\wCpo$-category, every
$\wCpo$-enriched, mixed-variance functor $F :
\opposite{\catD}\times\opposite{\catC}\times{\catD}\times\catC
\to \catC$ has a parameterised solution to the recursive equation
$\semroll : F(A, X, A', X) \xto{\isomorphic} X$, for every $A$, $A'$ in
$\catD$, namely the bilimit $\pair{\mu B.F(A,B,A',B)}{d_{F, A, A'}}$
of
\[
\Init \epto F(A, \Init, A'\!, \Init)
\epto F(A, F(A, \Init, A'\!, \Init), A'\!, F(A, \Init, A'\!, \Init)) \epto \cdots
% \epto F^n(A, A') \epto \cdots
\]
The solution is minimal in the sense of \cite{pitts1996relational}.  The
assignments $\mu B. F(A, B, A', B)$ extend to a mixed-variance functor
$\mu B. F(-, B, -, B) : \opposite{\catD}\times\catD \to \catC$
by $\mu B. F(f, B, g, B) := \vee_{n}\emb d_n\circ F^n(f,
g)\circ \prj d_n  $.

Finally, a \emph{bilimit compact expansion} $J : \catV \embed \catC$
is a triple consisting of an $\wCpo$-category $\catV$, a bilimit
compact category $\catC$; and an identity-on-objects, 
$\wCpo$-enriched order reflecting functor $J : \catV \to \catC$ such that,
for every ep-pair \wchain{}s $\pair Aa$, $\pair Bb$ in $\catC$,
their bilimits $\pair Dd$, $\pair Ee$, and countable collection of
$\catV$-morphisms $\seq[n \in \NN]{\alpha_n : A_n \to B_n}$ such
that for all $n$:
\[
J\alpha_{n+1} \circ \emb a_n = \emb b_n\circ J\alpha_n, \qquad  J\alpha_{n}\circ \prj a_n = \prj b_n\circ J\alpha_{n+1}
\]
(i.e., $J\alpha : \pair A{\emb a} \to \pair B{\emb b}$ and $J\alpha
: \pair A{\prj a} \to \pair B{\prj b}$ are natural transformations),
there is a $\catV$-morphism $f : D \to E$ such that $Jf = \vee_{n}
\emb e_n\circ \alpha_n \circ \prj d_n$. The motivation for
this definition: given two bilimit compact expansions $J' :
\catV' \embed \catC'$, $J : \catV \embed \catC$, and two
$\wCpo$-enriched functors \[ F : \opposite{\catV'}\times \opposite\catV \times \catV'
\times \catV \to \catV \quad G : \opposite{\catC'}\times
\opposite{\catC} \times \catC' \times \catC \to \catC
\quad\text{s.t.}\quad G\circ \opposite {J'}\times \opposite J \times J'
\times J = J\circ F
\]
the functor $\mu B. G(-, B, -, B) : \opposite{\catD}\times \catD
\to \catC$ restricts to $\mu B. G(\opposite J-, B, J-, B) :
\opposite{\catV}\times \catV \to \catV$.
Bilimit compact expansions are closed under small products, opposites,
and exponentiation with small categories~\cite{levy2012call}.


\subsubsection*{Type formers}
Suppose that we are given an $CBV$ $\wCpo$-pair $\left( \catV , \monadT \right) $ and let $J:\catV\to\catC$ be the corresponding $\catV$-enriched universal
Kleisli functor.
Suppose that it forms a bilimit compact expansion.

As usual, we interpret types $\ty{1}$ in kinding context $\Delta=\tvar{1}_1,\ldots,\tvar{1}_n$ 
as $\wCpo$-enriched functors $\sem{\ty{1}}:(\catC^{op}\times\catC)^n\to \catC $ that restrict to functors
$\sem{\ty{1}}_v:(\catV^{op}\times\catV)^n\to \catV $.
We interpret computations $\DGinf{\trm{1}}{\ty{1}}$ as dinatural transformations $\sem{\trm{1}}:\sem{\Gamma}\to \sem{\ty{1}}$
and values $\DGinf{\val{2}}{\ty{1}}$ as dinatural transformations $\sem{\val{2}}_v:\sem{\Gamma}_v\to \sem{\ty{1}}_v$.
\todo{spell out how.}

==> TEX/app-not-really-differentiable.tex <==
\section{AD transformation for non-differentiable functions}\label{app:not-really-diffentiable}





==> TEX/arrays.tex <==
\section{AD on arrays}\label{sec:arrays}
\todo{write something here about how arrays are the same as lists (included in recursive types),
semantically.
}
\todo{so: included in stronger correctness theorem}
\todo{explain how we can use array/list as return type for dual numbers reverse AD.}

==> TEX/beta-eta3.tex <==
\[
\begin{array}{l@{\ }l}
(\Lambda\tvar{1}.\trm{1})\,\ty{1}\beeq\subst{\trm{1}}{\sfor{\tvar{1}}{\ty{1}}}\qquad\qquad & \trm{1}\freeeq{\tvar{1}}\Lambda\tvar{1}.\trm{1}\,\tvar{1}
\end{array}    
\]


==> TEX/d-types-terms3.tex <==
\[
    \begin{array}{lll}
        \Dsynplain{\forall\tvar{1}.\tysch{1}} \defeq {\forall.\tvar{1}}.\Dsynplain{\tysch{1}}   \qquad
         & \Dsynplain{\Lambda\tvar{1}.\trm{1}}\defeq\Lambda\tvar{1}.\Dsynplain{\trm{1}}\qquad &\Dsynplain{\trm{1}\,\ty{1}}\defeq 
    \Dsynplain{\trm{1}}\,\Dsynplain{\ty{1}}
\end{array} 
    \]

==> TEX/extra.tex <==
\section{Currently unused material}

\subsection*{Untyped languages}
Remembering that we can consider a dynamically typed functional language as a sublanguage of a language 
with recursive types. 
Indeed, we can define the recursive type 
$$
\LTerm\defeq \trec{\tvar{1}}{\reals\t+\Unit\t+(\tvar{1}\t*\tvar{1})\t+\Init\t+(\tvar{1}\t+\tvar{1})\t+(\tvar{1}\To\tvar{1})}
$$
at which we can interpret all programs, following the recipe of \cite[\S2.3]{vakar2019domain}.
Seeing that we have a coercion 
$\Dsyn{\LTerm}\to \LTerm$,
we can now interpret $\Dsynsymbol$ as a code transformation from programs of type $\LTerm$ to programs of type $\LTerm$.
Our correctness theorem now justifies the use of dual numbers AD methods on dynamically typed functional languages such as Lisp-family languages. 

\todo{Honestly, I'm not sure we should bother with a section like this.}

\subsection*{Extending to polymorphism}
The AD techniques that we described in this paper are uniquely suited for application to expressive functional languages in the ML-family such as O'Caml and Haskell.
One feature of the type system of such languages beyond those that we have already described is the presence of (higher-order) polymorphism.

We can use a minor variation on the semantics $\sem{-}$ constructed so far, by replacing $\wCpo$ with the category of  Scott predomains (bounded-cocomplete algebraic directed-cocomplete partial orders) and directed-cocontinuous functions.
As described in  \cite[\S5.6]{crole1993categories}\footnote{In fact, the development in loc. cit. uses Scott domains, but all proofs apply equally if we work with Scott predomains. Care only needs to be taken in the proof of Theorem 5.6.6, where we need to define $\Omega$ as the one-point predomain $\set{*}$ instead, $\tilde{e}(*)=e$ and $p(l)=*$.}, this category additionally models (higher-order) polymorphism.
It is well-known that logical relations arguments, such as our correctness argument for AD, extend to polymorphism \cite[Proposition 18]{ma1991types}\footnote{Again, the development in loc. cit. is phrased in terms of admissible relations on Scott domains, but it applies equally to chain-complete relations on Scott predomains.
In fact, it is simpler as one does not need to check the strictness of various morphisms.}.
\todo{We should actually be a bit more careful about moving these results to CBV.
Honestly, it doesn't really seem worth it.}

==> TEX/operational-attempt <==
Well, the traditional CBV reduction rule for recursion is
\mu z. t , K --> let z = (\mu z.t) in t , K
So that's what we want to reproduce in some way.


CBPV with recursion has a well-defined operational semantics, right? So what we need is that the CBPV encoding of CBV recursion gives the standard CBV operational semantics for recursion.

\Gamma, x : U(A -> F B) |-^c t : FU(A -> FB) 
----------------------------------------------
\Gamma, z : UFU(A -> F B) |-^c force z to x.t : FU(A -> FB) 
----------------------------------------------
\Gamma |-^c mu z. force z to x.t : FU(A -> FB) 
----------------------------------------------
\Gamma |-^c (mu z. force z to x.t) to y. force y : A -> FB
----------------------------------------------
\Gamma |-^v thunk ((mu z. force z to x .t) to y. force y) : U(A -> FB)

this should be the encoding of CBV recursion as a value in CBPV.

The corresponding computation is therefore return (thunk ((mu z. force z to x .t) to y. force y)) .

For a general stack, this doesn't have the correct operational semantics.

Indeed, the configuration

return (thunk ((mu z. force z to x .t) to y. force y)) , K

doesn't reduce (gets stuck) unless K = (-) to yy. r :: L . That seems a bit bad at first.

However, if we think about it more, we only really care that 
(\mu z.t ) V 
and 
(let z = (\mu. t) in t) V
have a common redex 
as recursion is only ever used to define a function in CBV, which we need to apply to use it.

Then, the translation of (\mu z. t) V would be 

(return (thunk ((mu z. force z to x .t) to y. force y))) to xx. return V to yy. (force xx) yy

We'd want to show that 
(return (thunk ((mu z. force z to x .t) to y. force y))) to xx. return V to yy. (force xx) yy , K 
and
(return (thunk ((mu z. force z to x .t) to y. force y)) to x. t) to xx. return V to yy. (force xx) yy, K
have a common redex.

Now,
(return (thunk ((mu z. force z to x .t) to y. force y))) to xx. return V to yy. (force xx) yy , K 
-->
(return (thunk ((mu z. force z to x .t) to y. force y)))  , (-) to xx. return V to yy. (force xx) yy :: K 
-->
return V to yy. (force (thunk ((mu z. force z to x .t) to y. force y))) yy , K 
--> 
return V ,   (-) to yy . (force (thunk ((mu z. force z to x .t) to y. force y))) yy :: K
-->
(force (thunk ((mu z. force z to x .t) to y. force y))) V, K 
--> 
(force (thunk ((mu z. force z to x .t) to y. force y))), (-) V :: K 
--> 
((mu z. force z to x .t) to y. force y), (-) V :: K 
-->
mu z. force z to x .t , (-) to y. force y :: (-) V :: K     [Now we have reached the point of CBV recursion treated as a computation again]
--> (***) (see computation treatment below)
(\mu z. force z to x. t) ,  (-) to x. t :: (-) to y. force y :: (-) V :: K 
--> (not sure how to continue here)



The other configuration reduces as
(return (thunk ((mu z. force z to x .t) to y. force y)) to x. t) to xx. return V to yy. (force xx) yy, K 
-->
(return (thunk ((mu z. force z to x .t) to y. force y)) to x. t) ,(-) to xx. return V to yy. (force xx) yy :: K 
-->
(return (thunk ((mu z. force z to x .t) to y. force y))) , (-) to x. t :: (-) to xx. return V to yy. (force xx) yy :: K 
-->
t[(thunk ((mu z. force z to x .t) to y. force y))/x] , (-) to xx. return V to yy. (force xx) yy :: K 
--> (assuming t = return (thunk s))
return V to yy. (force (thunk s[(thunk ((mu z. force z to x .t) to y. force y))/x])) yy , K 
--> 
(force (thunk s[(thunk ((mu z. force z to x .t) to y. force y))/x]))  , (-) V :: K 
-->
s[(thunk ((mu z. force z to x .t) to y. force y))/x]  , (-) V :: K 


Meanwhile, the treatment of CBV recursion as a computation in CBPV is

\Gamma, x : U(A -> F B) |-^c t : FU(A -> FB)
-------------------------------------------------------------
\Gamma, z : UFU(A -> F B) |-^c force z to x.t : FU(A -> FB)
-------------------------------------------------------------
\Gamma |-^c mu z. force z to x .t : FU(A -> FB)

We need to show that 

\muCBV z .t , K 
and
let z = (\muCBV z. t) in t, K
have a common redex

That is
\mu z. force z to x. t, K
and 
(\mu z. force z to x. t) to x. t , K
have a common redex

Supposing that we can show that. Then the step (***) in our CBV recursion as value treatment above works as well.

Now, 
\mu z. force z to x. t, K
-->
(force z to x. t)[\mu z. force z to x. t/z], K
-->
(force (thunk (\mu z. force z to x. t))) to x. t, K
-->
(force (thunk (\mu z. force z to x. t))) , (-) to x. t :: K
-->
(\mu z. force z to x. t) , (-) to x. t :: K

and 

(\mu z. force z to x. t) to x. t , K
-->
(\mu z. force z to x. t) , (-) to x. t :: K
(Yay!)






(\mu z. force z to x. t) to xx. return V to yy. (force xx) yy , K
-->
(\mu z. force z to x. t) ,(-) to xx. return V to yy. (force xx) yy :: K
-->
(\mu z. force z to x. t) , (-) to x. t :: (-) to xx. return V to yy. (force xx) yy :: K













\Gamma, x : A -> B |-^c t :  A -> B 
------------------------------------------------
\Gamma, x : A -> B, z : A |-^c t to x. x z : B
------------------------------------------------
\Gamma, x : A -> B |-^v \z:A . t to x. x z : A -> B
------------------------------------------------
\Gamma |-^v \mu x.\z:A.t to x. x z : A -> B 
----------------------------------------------
\Gamma |-^c return \mu x.\z:A.t to x. x z : A -> B 

==> TEX/polymorphism.tex <==
\section{ML-style polymorphism}\label{sec:polymorphism}
We extend our language with ML-style polymorphism.

\subsection{Syntax}
That is, we extend our syntax as \\
\input{types-values-computations3}\\
The important part is that we distinguish between types (which may not contain universal quantification) and type schemas (which may), which allows us to avoid impredicative 
quantification.
In particular, universal quantification always occurs at the very outside of a type scheme.
Figure \ref{fig:types3} lists the standard typing rules for polymorphic types.
We use these on top of the typing rules of Figure \ref{fig:types1} and \ref{fig:types2}.


\begin{figure}[!ht]
	\fbox{\parbox{0.98\linewidth}{\begin{minipage}{\linewidth}\noindent\input{type-system3}\end{minipage}}}
	\caption{Typing rules for ML-style polymorphism. 
		\label{fig:types3}}
\end{figure}
We consider the standard equations of Figure \ref{fig:beta-eta3}.
\begin{figure}[!ht]
	\fbox{\parbox{0.98\linewidth}{\scalebox{0.92}{\begin{minipage}{\linewidth}\noindent\input{beta-eta3}\end{minipage}}}
	}\caption{\label{fig:beta-eta3} the standard $\beta\eta$-rules for polymorphism.
	}
\end{figure}


\subsection{Automatic differentiation}
Figure \ref{fig:ad3} lists our rules for differentiating polymorphic programs.
\begin{figure}[!ht]
	\fbox{\parbox{0.98\linewidth}{\begin{minipage}{\linewidth}\noindent
				\input{d-types-terms3}
	\end{minipage}}}
	\caption{The definitions of AD on polymorphism, where $\Dsynplainsymbol=\Dsynsymbol$ or $\Dsynplainsymbol=\Dsynrevsymbol[k]$. \label{fig:ad3}}
\end{figure}

\subsection{Semantics}
As before, we interpret type schemas $\tysch{1}$ with free type variables $\tvar{1}_1,\ldots,\tvar{1}_n$ as functors $\sem{\tysch{1}}:(\wCpo^{op}\times \wCpo)^n\to \wCPO$, where we
 write $\wCPO$ for the category of large \wcpos{} and monotone \wcont{} functions.
This category has all large $\wCPO$-enriched limits.
We can therefore define the end 
$$
\sem{\forall\tvar{1}_n.\tysch{1}}\defeq \int_a \sem{\tysch{1}}(-,\ldots,-,(a,a)):(\wCpo^{op}\times \wCpo)^{n-1}\to \wCPO.
$$
We interpret 


\todo{describe end semantics, giving large wcpos}

\subsection{Logical relations and AD correctness}
\todo{describe definition of category of large logical relations and how to compute ends there}

==> TEX/reverse-ad.tex <==
\section{Dual numbers reverse AD}\label{sec:reverse-ad}
We can implement a reverse AD algorithm using a minor variation of the 
dual numbers forward AD technique we have discussed so far.
By using a custom operational semantics for linear functions, \cite{brunel2019backpropagation}  
proved that this algorithm has the correct computational complexity. 
Recently, \cite{smeding2022} proposed a practical implementation technique and showed that it scaled to 
an elegant and efficient AD algorithm that differentiates most of Haskell98.

\subsection{Extending the target language}
To support reverse AD, we implement the target language of our code transformation 
as a slight extension of the source language.

The idea is that $\reals\multimap\reals^n$ behaves like the function type $\reals\To\reals^n$ except that we are free to use a more efficient operational semantics that makes smart use of linearity of the functions to speed up evaluation: $(\lincomp{\trm{1}}{\trm{2}})\plus (\lincomp{\trm{1}}{\trm{3}})$ gets evaluated as $\lincomp{\trm{1}}{(\trm{2}+\trm{3})}$.


\subsection{Code transformation}
By setting $\Dsynrev[k]{\reals}\defeq \reals\t*(\reals\multimap\reals^k)$ and replacing the uses of $\cnst{0}$ by $\zero$, $+$ by $\plus$, and $*$ by $\lincomp{}{}$ in $\Dsynsymbol$, we get the code transformation $\Dsynrevsymbol[k]$ for reverse AD.
\todo{add wrapper?
also, should we bring in some the details from the key ideas section?
}

\subsection{Semantics and correctness statement}
We interpret $\sem{\reals\multimap\reals^k}\defeq \RR\multimap \RR^k$ as the space of $\RR$-vector space homomorphisms.
Then,
\begin{align*}
    \sem{\biprodin{i}}&\defeq r\mapsto (\overbrace{0,\ldots,0}^{i-1},r,\overbrace{0,\ldots 0}^{k-i})
    &\sem{\zero} & \defeq r\mapsto \overbrace{(0,\ldots,0)}^k\\
    \sem{\trm{1}\plus\trm{2}} & \defeq r\mapsto \sem{\trm{1}}(r)+\sem{\trm{2}}(r)
    &\sem{\lincomp{\trm{1}}{\trm{2}}} & \defeq r\mapsto \sem{\trm{1}}(\sem{\trm{2}}*r).
\end{align*}
This lets us state the correctness theorem.
\todo{copy statement from key ideas? we need to probably state certain things in key ideas and just refer to them here rather than copying. or we should only be vague in key ideas and then state them here.}

\subsection{Logical relations and correctness proof}
\todo{here, give categorical proof?
}



==> TEX/type-system-target-1.tex <==
\[
  \begin{array}{c}
\inferrule{
  \Ginf{\trm{1}}{\tangreals{k}}\quad
  \Ginf{\trm{2}}{\tangreals{k}}\quad \left( k\in \FinDimS\right) 
}{
  \Ginf{\trm{1} + \trm{2} }{\tangreals{k}}
}
\quad 
\inferrule{
	\Ginf{\trm{1}}{\tangreals{k}}\quad
	\Ginf{\trm{2}}{\tangreals{k}}\quad \left( k\in \FinDimS\right) 
}{
	\Ginf{\trm{1} + \trm{2} }{\tangreals{k}}
}
\quad
\inferrule{ (c\in\RR)}{\Ginf {\cnst{c}}\reals}\\ \\
   \inferrule{
     \set{\Ginf {\trm{1}_1} \reals}_{i=1}^n\quad (\op\in\Op_n)
   }{
     \Ginf {\op(\trm{1}_1,\ldots,\trm{1}_n)}\reals
   }
\quad 
\inferrule{\Ginf{\trm{1}}\Init}{\Ginf {\nvMatch{\trm{1}}}{\ty{1}}}\quad 
   \quad
   \inferrule{\Ginf {\trm{1}} {\ty{1}}}
   {\Ginf{\tInl\trm{1}}\ty{1}\t+\ty{2}}
   \\\\
   \inferrule{\Ginf {\trm{1}} {\ty{1}}}
   {\Ginf{\tInr\trm{1}}\ty{1}\t+\ty{2}}
   \quad
   \inferrule{\Ginf{\trm{3}}{\ty{2}\t+\ty{3}}\quad
   \Ginf[,\var{1}:\ty{2}]{\trm{1}}{\ty{1}}\quad 
   \Ginf[,{\var{2}}:\ty{3}]{\trm{2}}{\ty{1}}
   }{\Ginf{\bvMatch{\trm{3}}{\var{1}}{\trm{1}}{\var{2}}{\trm{2}}}{\ty{1}}}
   \quad 
   \inferrule{~}{\Ginf \tUnit \Unit}\\ \\ 
   \inferrule{\Ginf {\trm{1}} {\ty{1}}\quad \Ginf {\trm{2}} {\ty{2}}}
   {\Ginf {\tPair{\trm{1}}{\trm{2}}} {\ty{1}\t*\ty{2}}}
   \quad 
   \inferrule{
   \Ginf {\trm{3}}{\ty{2}\t*\ty{3}}\quad 
   \Ginf[{,\var{1}:\ty{2},\var{2}:\ty{3}}] {\trm{1}}{\ty{1}}}{\Ginf{\pMatch{\trm{3}}{\var{1}}{\var{2}}{\trm{1}}}{\ty{1}}}
   \quad 
   \inferrule{\Ginf[,\var{1}:{\ty{2}}]{\trm{1}}{\ty{1}}}{\Ginf{\fun{\var{1}}{\trm{1}}}{\ty{2}\To\ty{1}}} \\ \\ 
   \inferrule{\Ginf {\trm{1}} {\ty{2}\To\ty{1}}
   \quad\Ginf {\trm{2}}{\ty{2}} 
   }{\Ginf {\trm{1}\,\trm{2}}{\ty{1}}}
   \quad 
  \inferrule{\Ginf[,\var{1}:{\ty{2}}] {\trm{1}}{\ty{2}\t+\ty{1}}
   \quad \Ginf {\trm{3}} {\ty{2}} }{\Ginf {\tItFrom{\trm{1}}{\var{1}}{\trm{3}}}{\ty{1}}}
   \\\\
   \inferrule{ \Ginf[,\var{1}:\ty{1}]{\trm{1}}{\ty{1}}}
   {\Ginf{\rec{\var{1}}{\trm{1}}}{\ty{1}}}(\ty{1}=\ty{2}\To\ty{3})
   \quad
   \inferrule{\Ginf {\trm{3}} \reals}{\Ginf {\tSign\trm{3}} {\Unit\t+ \Unit}
   }
\end{array}
\]


==> TEX/type-system3.tex <==
\[
  \begin{array}{c}
\inferrule{
  \Delta,\tvar{1}\mid\Ginf{\trm{1}}{\tysch{1}}
}{
  \Delta \mid \Ginf {\Lambda \tvar{1}.\trm{1}}{\forall\tvar{1}.\tysch{1}}
}\qquad\qquad 
\inferrule{\Delta\mid \Ginf{\trm{1}}{\forall\tvar{1}.\tysch{1}}
\quad 
\Delta\vdash \ty{1}\,\type
}
{\Delta\mid \Ginf{\trm{1}\,\ty{1}}{\subst{\tysch{1}}{\sfor{\tvar{1}}{\ty{1}}}}}
\end{array}
\]


==> TEX/types-values-computations-target.tex <==
\begin{syntax}
    \ty{1}, \ty{2}, \ty{3} & \gdefinedby & & \syncat{types}                          \\
    &\gor& \reals                      & \synname{numbers}\\
    &\gor & \Init  \gor \ty{1} \t+ \ty{2}  & \synname{sums}\\
    &&&\\
    \val{1}, \val{2}, \val{3} & \gdefinedby & & \syncat{values}                          \\
    &\gor& \var{1},\var{2},\var{3}                      & \synname{variables}\\
    &\gor& \cnst{c}                   & \synname{constants}\\
    &\gor& \tInl{\val{1}} \gor   \tInr{\val{1}} & \synname{sum inclusions}\\
    &&&\\
    \trm{1}, \trm{2}, \trm{3} & \gdefinedby & & \syncat{computations}                          \\
    &\gor& \var{1},\var{2},\var{3}                      & \synname{variables}\\
    &\gor & \letin{\trm{1}}{\var{1}}{\trm{2}} & \synname{sequencing}\\
    &\gor& \cnst{c}                   & \synname{constant}\\
    &\gor & \op(\trm{1}_1,\ldots,\trm{1}_n) & \synname{operation}\\
    &\gor & \nvMatch{\trm{1}} & \synname{sum match}\\
	&\gor& \tInl{\trm{1}} \gor   \tInr{\trm{1}} & \synname{sum inclusions}\\
    &\gor & \vMatch{\trm{3}}{\begin{array}{l}\;\;\tInl\var{1}\To\trm{1}\\
    \gor \tInr\var{2}\To \trm{2}\end{array}}\hspace{-15pt}\; & \synname{sum match}\\
  \end{syntax}%
~
 \begin{syntax}
	&\gor\quad\, & \Unit  \gor  \ty{1}_1 \t* \ty{1}_2 & \synname{products}\\
  &\gor& \ty{1} \To \ty{2}              & \synname{function}      \\
	& & &\\
	&&&\\
	&\gor\quad\, & \tUnit \ \gor  \tPair{\val{1}}{\val{2}} & \synname{tuples}\\
  &\gor& \fun{\var{1}}{\trm{1}}             & \synname{abstractions}      \\
  &\gor &\rec{\var{1}}{\trm{1}} & \synname{term recursion}\\
  &&&\\\\
	&\gor\quad\, & \tUnit \ \gor  \tPair{\trm{1}}{\trm{2}} & \synname{tuples}\\
	% &\gor\quad\, & \uMatch{\trm{2}}{\trm{1}} & \synname{product match}\\
	&\gor\quad\, & \pMatch{\trm{2}}{\var{1}}{\var{2}}{\trm{1}}\hspace{-10pt}\; & \synname{product match}\\
	&\gor& \fun{\var{1}}{\trm{1}}             & \synname{abstractions}      \\
	&\gor& \trm{1}\ \trm{2}             & \synname{function app.}      \\
	&\gor&\tItFrom{\trm{1}}{\var{1}}{\trm{2}}\hspace{-10pt}\; & \synname{iteration}\\
	& \gor & \rec{\var{1}}\trm{1} & \synname{term recursion}\\
	&\gor&\tSign\trm{1} & \synname{sign function}
\end{syntax}

==> TEX/types-values-computations-termrecursion.tex <==
\begin{syntax}
    \ty{1}, \ty{2}, \ty{3} & \gdefinedby & & \syncat{types}                          \\
    &\gor& \reals                      & \synname{numbers}\\
    &\gor & \Init  \gor \ty{1} \t+ \ty{2}  & \synname{sums}\\
    &&&\\
    \val{1}, \val{2}, \val{3} & \gdefinedby & & \syncat{values}                          \\
    &\gor& \var{1},\var{2},\var{3}                      & \synname{variables}\\
    &\gor& \cnst{c}                   & \synname{constants}\\
    &\gor& \tInl{\val{1}} \gor   \tInr{\val{1}} & \synname{sum inclusions}\\
    &&&\\
    \trm{1}, \trm{2}, \trm{3} & \gdefinedby & & \syncat{computations}                          \\
    &\gor& \var{1},\var{2},\var{3}                      & \synname{variables}\\
    &\gor & \letin{\trm{1}}{\var{1}}{\trm{2}} & \synname{sequencing}\\
    &\gor& \cnst{c}                   & \synname{constant}\\
    &\gor & \op(\trm{1}_1,\ldots,\trm{1}_n) & \synname{operation}\\
    &\gor & \nvMatch{\trm{1}} & \synname{sum match}\\
	&\gor& \tInl{\trm{1}} \gor   \tInr{\trm{1}} & \synname{sum inclusions}\\
    &\gor & \vMatch{\trm{3}}{\begin{array}{l}\;\;\tInl\var{1}\To\trm{1}\\
    \gor \tInr\var{2}\To \trm{2}\end{array}}\hspace{-15pt}\; & \synname{sum match}\\
  \end{syntax}%
~
 \begin{syntax}
	&\gor\quad\, & \Unit  \gor  \ty{1}_1 \t* \ty{1}_2 & \synname{products}\\
  &\gor& \ty{1} \To \ty{2}              & \synname{function}      \\
	& & &\\
	&&&\\
	&\gor\quad\, & \tUnit \ \gor  \tPair{\val{1}}{\val{2}} & \synname{tuples}\\
  &\gor& \fun{\var{1}}{\trm{1}}             & \synname{abstractions}      \\
  &\gor &\rec{\var{1}}{\trm{1}} & \synname{term recursion}\\
  &&&\\\\
	&\gor\quad\, & \tUnit \ \gor  \tPair{\trm{1}}{\trm{2}} & \synname{tuples}\\
	% &\gor\quad\, & \uMatch{\trm{2}}{\trm{1}} & \synname{product match}\\
	&\gor\quad\, & \pMatch{\trm{2}}{\var{1}}{\var{2}}{\trm{1}}\hspace{-10pt}\; & \synname{product match}\\
	&\gor& \fun{\var{1}}{\trm{1}}             & \synname{abstractions}      \\
	&\gor& \trm{1}\ \trm{2}             & \synname{function app.}      \\
	&\gor&\tItFrom{\trm{1}}{\var{1}}{\trm{2}}\hspace{-10pt}\; & \synname{iteration}\\
	& \gor & \rec{\var{1}}\trm{1} & \synname{term recursion}\\
	&\gor&\tSign\trm{1} & \synname{sign function}
\end{syntax}

==> TEX/types-values-computations3.tex <==
\begin{syntax}
    \tysch{1}, \tysch{2}, \tysch{3} & \gdefinedby & & \syncat{type schemas}                          \\
    &\gor& \ty{1}                      & \synname{types}\\
    \\
    \val{1},\val{2},\val{3} & \gdefinedby && \syncat{values}\\
    &\gor&\ldots&\synname{as before}\\
    \\
    \trm{1},\trm{2},\trm{3} & \gdefinedby && \syncat{computations}\\
    &\gor&\ldots&\synname{as before}\\
  \end{syntax}%
~
 \begin{syntax}
  &\gor\quad\, & \forall\tvar{1}.\tysch{1} & \synname{universal quantification}\\
  \\
  \\
  &\gor & \Lambda\tvar{1}.\trm{1} & \synname{polymorphic function}\\
  \\\\
  &\gor & \Lambda\tvar{1}.\trm{1} & \synname{polymorphic function}\\
  &\gor & \trm{1}\,\ty{1} & \synname{instantiation}
\end{syntax}

==> TEX/wCPO-enriched-subscone.tex <==
\section{Enriched subscone}\label{app-wCPO-enriched-subscone}



